Reshaping Convex Polyhedra

Given a convex polyhedral surface P, we define a tailoring as excising from P a simple polygonal domain that contains one vertex v, and whose boundary can be sutured closed to a new convex polyhedron via Alexandrov's Gluing Theorem. In particular, a digon-tailoring cuts off from P a digon containing v, a subset of P bounded by two equal-length geodesic segments that share endpoints, and can then zip closed. In the first part of this monograph, we primarily study properties of the tailoring operation on convex polyhedra. We show that P can be reshaped to any polyhedral convex surface Q a subset of conv(P) by a sequence of tailorings. This investigation uncovered previously unexplored topics, including a notion of unfolding of Q onto P--cutting up Q into pieces pasted non-overlapping onto P, and to continuously folding P onto Q. In the second part of this monograph, we study vertex-merging processes on convex polyhedra (each vertex-merge being in a sense the reverse of a digon-tailoring), creating embeddings of P into enlarged surfaces. We aim to produce non-overlapping polyhedral and planar unfoldings, which led us to develop an apparently new theory of convex sets, and of minimal length enclosing polygons, on convex polyhedra. All our theorem proofs are constructive, implying polynomial-time algorithms.

==> Punfoldings_2Jul2021.tex <==
\chapter{Enlarging and $P$-Unfoldings}
\chaplab{Punfoldings}

In this chapter we show how to enlarge a convex polyhedron $Q$ to some $P \supset Q$, via tailoring. 
Based on this operation, we introduce the notion of a $P$-unfolding and propose a few methods to accomplish it.

\section{Enlarging and Reshaping}
Previous chapters have established three methods of tailoring $P$ to $Q$:
\begin{itemize}
\squeezelist
\item Theorem~\thmref{MainTailoring}: For $Q \subset P$, digon-tailor following a sculpting of $P$ to $Q$.
\item Theorem~\thmref{CrestTailoring}: For $Q \subset P$, crest-tailor following a sculpting of $P$ to $Q$.
\item Theorem~\thmref{TailoringFlattening}:  via flattening, digon-tailor $P$ to a (possibly small) homothet of $Q$.
\end{itemize}
If we do not have $Q \subset P$, then shrinking $Q$ until it can fit in $P$ leads
to a homothet of $Q$. 
All three approaches result in the homothet of $Q$ being composed entirely of $P$-surface.
In the tailoring-via-flattening algorithm, $Q$ is enlarged with vertex-merging inserts,
but the last steps remove all inserts.
%, so again the $Q$-homothet is composed of $P$-surface.
%\blue{[Removed ``so again the $Q$-homothet is composed of $P$-surface."
%Actually, the inserts are composed entirely of $P$-surface. They are new surface when
%$Q$ is enlarged, but later all is $P$-surface. Confusing.]}

\medskip

In this short chapter, we explore some results that can be achieved through a mix
of vertex-merge enlarging, and tailoring. Part~II will explore vertex-merging
more thoroughly.

Suppose $Q \subset P$. Then we can enlarge $Q$ to $P$
using any one of the three tailoring algorithms, as follows.
We first tailor $P$ to $Q$, tracking the cuts and digons % of $P$-surface 
removed.
For crest-tailoring, we cut the boundary of crests.
Then, starting with $Q$, we cut each sealed geodesic or crest-boundary
and insert the earlier removed corresponding digon 
or crest surface, in reverse order.
The result is that $Q$ is enlarged by the surface insertions 
(of $P$-surface)
in the reversing process
until it matches $P$.

If $Q \not\subset P$, so $P$ and $Q$ are of arbitrary relative sizes,
we can reshape $P$ to $Q$ by 
first enlarging $P$ to
some $P' \supset Q$ large enough to enclose $Q$, 
and then tailor $P'$ to $Q$.
Here $P'$ is an arbitrary polyhedron midway in the process
$P \to P' \to Q$; it only needs to be large enough.

These enlargings can be accomplished within the same $O(n^4)$ time complexity
of the tailoring algorithms.
And in analogy with Corollary~\lemref{approx_tailoring},
enlargings of $Q$ can approximate any target surface $S$.
%\blue{[Joined previous two 1-sentence paragraphs.]}

We summarize the above discussion in a theorem:

\begin{thm}
\thmlab{Enlarge}
Let $P$ and $Q$ be convex polyhedra.
If $Q \subset P$, $Q$ may be enlarged with surface insertions to $P$.
If $Q \not\subset P$, $P$ can be reshaped to $Q$ with a combination of
surface insertions and excisions.
Either process can be accomplished in time $O(n^4)$,
and can approximate non-polyhedral convex surfaces.
\end{thm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{$P$-unfoldings}
\seclab{Punfoldings}


For $Q \subset P$, we can view the enlarging of $Q$ to $P$ just described
as ``unfolding" $Q$ onto $P$. We call this a \emph{$P$-unfolding of $Q$}.
To our knowledge, this notion has never been considered before.
We explore it  briefly here, and in more detail in Part~II.


\subsection{$P$-unfoldings and Reshaping}
\seclab{PunfReshaping}
%As a direct consequence of Section~\secref{Enlarging}, we can answers positively the following problem, apparently not previously explored.
Unfoldings of convex polyhedra to a plane have been studied extensively;
see, e.g., \cite{do-gfalop-07}.
Particular attention has been paid to unfolding to few pieces,
to connected unfoldings, and to non-overlapping unfoldings.
Often the goal is to achieve a \emph{net}, an unfolding to a single, simply connected, non-overlapping polygon in the plane.

Instead of unfolding a convex polyhedron $Q \subset P$ to a plane,
consider the question: 
Can one cut-up the surface $Q$ so that the pieces may be pasted onto $P$, non-overlapping,
and so form an isometric subset of $P$? 
This is a \emph{$P$-unfolding of $Q$}, or \emph{an unfolding of $Q$ onto $P$}.
It can be achieved via enlarging:
just enlarge $Q$ to $P$, and then remove all inserted digons or crests.
The result is a subset of $P$ isometric to the cut-up $Q$.
Note that all three enlarging methods retain the entire surface of $Q$---the enlarging
is accomplished by insertions of surface not part of $Q$.

This viewpoint incidentally yields a different proof of this known result:

\begin{co}
\thmlab{Areas}
Given convex polyhedra $P$ and $Q \subset P$, the area of $Q$ is smaller than the area of $P$.
\end{co}

%\begin{thm}
%\thmlab{thmP-unf}
%Given convex polyhedra $P$ and $Q$ of at most $n$ vertices each, and $Q \subset P$, a $P$-unfolding of $Q$ can be determined in time $O(n^4)$, following 
%Theorem~\thmref{Enlarge_Algorithm1}.
%\end{thm}
%
%\begin{proof}
%Just enlarge $Q$ to $P$, and then remove all inserted digons or crests.
%The result is a subset of $P$ isometric to the cut-up $Q$.
%\end{proof}
%
%\red{[The following is a direct corollary of, and should be put right after, Theorem~\thmref{Enlarge_Algorithm1}.]}
%\blue{[Moved to here; later will move to right spot.]}
%Theorem~\thmref{Enlarge_Algorithm1} provides another proof of this known result:
%
%\begin{co}
%\thmlab{areas_ineq}
%Given convex polyhedra $P$ and $Q \subset P$, the area of $Q$ is smaller than the area of $P$.
%\end{co}


To justify the use of the term ``unfolding," we describe an example of a simply connected $P$-unfolding embedding that does not achieve a net when unfolded to a plane.
Let $Q$ be the classical thin, nearly flat tetrahedron with an overlapping edge-unfolding.
See, e.g., \cite[Fig.~22.8, p.~314]{do-gfalop-07}.
Take $P$ to be a slightly larger homothet of $Q$.
Then the same edge-cuts that result in overlap in the plane embed $Q$ onto $P$ without overlap.
In a sense, it can be easier in some cases to unfold to $P$ than to unfold to a plane.

One focus of interest in the unfolding literature is the ``fewest nets" 
problem~\cite[Prob.~22.1, p.~308]{do-gfalop-07}: 
edge-unfold a polyhedron into the fewest number of nets.
Of course one net would be ideal, but it is a long-standing
open problem to determine if every convex polyhedron can be edge-unfolded
to a net---D{\"u}rer's problem~\cite{o-dp-13}.
This suggests it could be of interest 
to minimize the number of disconnected pieces of a $P$-unfolding
of $Q$, a goal we pursue in Part~II.
See also Open Problem~\openref{PunfConnected}.


\paragraph{Example: Hexagon inscribed in a triangle.}
Let $P$ be a doubly-covered triangle $abc$, and $Q$ a 
doubly-covered hexagon inscribed in $P$,
as in Fig.~\figref{HexInTri}.
Digon-tailoring $P$ to $Q$ is achieved by excising the vertices $a,b,c$ by
cutting digons bounded by the hexagon edges
$e_1,e_2,e_3$ respectively, and then sealing the cuts closed.
To enlarge $Q$ to $P$ by reversing the process,
each of those three edges is slit open and the pair of triangles
earlier removed is sutured back along the slit edges.
To obtain a $P$-unfolding, we simply skip inserting the pair of triangles.
The result is a ``pasting" of the two hexagons inside the two triangular faces of $P$.

Note that, to reverse a sealed digon, the resulting geodesic $\g$ is slit,
but the cut does not delete the endpoints $x_1,x_2$  of $\g$, as depicted in Fig.~\figref{DigonReverse}.
In other words, $\g \setminus \{x_1,x_2\}$ is doubled
to reproduce the digon boundary, but there remains one copy each of the $x_1,x_2$ endpoints.

Notice that each split $e_i$ is |blue{a} non-contractible closed curve inside the image of $Q$, so the embedding
of $Q$ onto $P$ in this case is not simply connected: it has three holes.

%see Fig.~\figref{HexInTri}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Figure Begin
\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\linewidth]{Figures/Punfoldings/HexInTri}
\caption{Doubly-covered hexagon $Q$ inscribed inside / enlarged to a doubly-covered triangle $P$.}
\figlab{HexInTri}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Figure End
\qquad %Force figs on same page
%see Fig.~\figref{DigonReverse}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Figure Begin
%\begin{figure}[htbp]
\centering
\includegraphics[width=0.35\linewidth]{Figures/Punfoldings/DigonReverse}
\caption{Digon $x_1 x_2$ closes to geodesic $\g$.}
\figlab{DigonReverse}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Figure End


\medskip

The previous example shows
that the $P$-unfolding of $Q$ produced by enlarging is not necessarily simply connected.\footnote{
Notice that we do not require path-connectivity for the definition of simple connectivity.}
However, in general, that is indeed the case, as shown by the following result. 
We next explain the meaning of ``in general.''

\medskip

Consider the space ${\cal S}$ of all convex surfaces, endowed with the topology induced by the usual Pompeiu-Hausdorff metric.
Fix some $P \in {\cal S}$.
Consider in ${\cal S}$ the subset ${\cal P}={\cal P}_P^n$ of all polyhedra $Q\subset P$ with 
precisely $n$ vertices, with the induced topology.
Two polyhedra in ${\cal P}$ are then close to each other if and only if they have close 
corresponding vertices.
``General'' refers to polyhedra $Q$ in an open and dense subset of ${\cal P}$.

\begin{thm}
\thmlab{QPflat}
For any convex polyhedron $P$ and any $n \in \N$, there exists a subset ${\cal Q}={\cal Q}_P^n$ open and dense in ${\cal P}$, 
such that the $P$-unfolding $Q_P$ of each $Q \in {\cal Q}$ is flat (i.e., contains no internal vertices), and is simply connected.
\end{thm}

\begin{proof}
Assume we have some convex polyhedron $Q \subset P$ such that $Q_P$ contains an internal vertex $v$, and so the curvatures of $P$ and $Q$ at $v$ are equal: $\o_Q(v)=\o_P(v)$.
Slightly alter the position of the vertices of $Q$, to get $\o_Q(w) \neq \o_P(u)$, for any vertices $w \in Q$ and $u \in P$.
Of course, this remains valid in a small neighborhood of the new $Q$.

Assume now we have some convex polyhedron $Q \subset P$ such that $Q_P$ is not simply connected, 
i.e., $Q_P$ contains a noncontractible curve $\s \subset P \cap Q_P$.
The Gauss-Bonnet Theorem shows that the total curvature $\Omega_Q (\s)$ of $Q_P$ inside $\s$ equals the total curvature $\Omega_P (\s)$ of $P$ inside $\s$: $\Omega_Q (\s) = \Omega_P (\s)$. We next show that every such $Q$ that violates the theorem can be approximated with polyhedra that do satisfy the theorem.

Slightly alter the position of the vertices of $Q$, to get a new polyhedron $Q'$ on which the following property (V) is verified. 
(V): any partial sum of vertex curvatures is different from any partial sum of vertex curvatures in $P$. 
This implies that,  for any simple closed curve $\t$ on $Q'$, $\Omega_{Q'} (\t)$ cannot be written as the sum of vertex curvatures of $P$.
Therefore, $Q'_P$ has no curve in common with $P$, noncontractible in $Q'_P$. And so $Q'$ does satisfy the theorem.

Since the property (V) is valid on a neighborhood $N$ of $Q'$, it follows that all polyhedra in $N$ do satisfy the theorem.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{$P$-unfoldings and the Wallace-Bolyai-Gerwien Theorem}
\subsection{$P$-unfoldings and the WBG Theorem}

In this section we show that the $P$-unfolding question can also be answered by applying the 
powerful hinged variant of Wallace-Bolyai-Gerwien dissection theorem.
However, this will result in a ``pseudopolynomial number of pieces" and 
pseudopolynomial running time~\cite{abbott2012hinged}.\footnote{
They define pseudopolynomial as follows:
``pseudopolynomial means polynomial in the combinatorial complexity ($n$) and the dimensions of an integer grid on which the input is drawn."}

The Wallace-Bolyai-Gerwien (WBG) Theorem states that any two simple polygons with equal area can be dissected into finitely many simple congruent polygons.
It was strengthened in 
the paper, ``Hinged Dissections Exist"~\cite{abbott2012hinged},
where it is shown that the pieces can be chosen in an arcwise-connected chain, 
i.e., the dissection can be hinged at vertices along that chain.

\begin{thm}
\thmlab{WBG_Punf}
Given convex polyhedra $P$ and $Q$ of at most $n$ vertices each, and $Q \subset P$, a connected $P$-unfolding of $Q$ can be determined in pseudopolynomial number of pieces  and pseudopolynomial running time, following the WBG theorem and the hinge-dissection.
\end{thm}

\begin{proof}
We start with a quote from~\cite{abbott2012hinged}:
\begin{quotation}
\noindent
``One interesting consequence of [our] theorem is that any finite set of polyhedral surfaces of equal surface area have a common hinged dissection: It is known that every polyhedral surface can be triangulated and then vertex-unfolded into a hinged chain of triangles~\cite{deeho-vusm-03}. Our results (specifically Theorem~6) show how to construct a single hinged chain that can fold into any finite set of such chains, which can then be folded (and glued) into the polyhedral surfaces.''
\end{quotation}

\noindent A \emph{vertex-unfolding} of a triangulated polyhedron
is a chain of triangle connected at vertices. A vertex-unfolding
of a triangulated cube is shown in Fig.~\figref{VertexUnf}.

Let $A_Q$ and $A_P$ be the areas of $Q$ and $P$.
Triangulate and vertex-unfold both $P$ and $Q$.
The plan is to show that $A_Q$ can ``fit" exactly within
a sequence of $P$'s triangles, with at most one of $P$'s triangles
partitioned into two triangles.

Denote by $T_1,...,T_m$ the triangles in the chain corresponding to $P$, and by  $a_j$ denote the area of the $T_j$, $j=1,...,m$.
So we have $A_Q<A_P= \sum_{j=1}^m a_j$.
Then there exists $1 \leq h \leq m$ such that $a_1+...+a_{h-1} \leq A_Q < a_1+...+ a_h$.
Triangle $T_h$ is then the transitional triangle with respect to area in the sequence
of triangles.

%see Fig.~\figref{VertexUnf}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Figure Begin
\begin{figure}[htbp]
\centering
\includegraphics[width=1.0\linewidth]{Figures/Punfoldings/VertexUnf}
\caption{Area $A_Q$ (shaded) in vertex-unfolding of a triangulated cube.
$T_h=xyz$.
Based on Fig.2(a) in~\protect\cite{deeho-vusm-03}.}
\figlab{VertexUnf}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Figure End

Now we further dissect the triangle $T_h$ into two parts, one of which has area $c=A_Q - (a_1+...+a_{h-1})$.
Specifically, let $T_h = xyz$ and choose a point $w \in yz$ such that $|w-y|/|z-y| = c/a_h$.
Then the area $A'$ of the triangle $xyw$ is equal to $c/a_h$ of the area of $T_h$ (because both triangles have the same altitude through $x$).

Therefore, in the chain of triangles obtained from $P$, we can find an arcwise-connected subchain of total area equal to %the area of $Q$,
$A_Q$, possibly after partitioning one triangle.

Then Theorem~6 in~\cite{abbott2012hinged} constructs a single
hinged dissection chain of the triangles forming $Q$
into the triangles up to $T_h$ of $P$.
Then the $Q$-chain triangles can be placed inside the $P$-chain triangles,
achieving a connected $P$-unfolding of $Q$.

The ``pseudopolynomial number of pieces" and pseudopolynomial running
time follows from~\cite{abbott2012hinged}.
\end{proof}
\noindent
Note that although the $P$-unfolding constructed in this theorem's proof
is connected, its interior is not connected.

%\blue{[I am unclear if having a disconnected interior means it is not simply connected.
%I think it is simply connected because still any simple closed curve can be
%contracted. A curve through a vertex connection would not be a simple curve.
%I don't know what term should be used for ``connected interior." Maybe there is
%no accepted term aside from ``connected interior."]}
%\red{[I agree with both your comments.]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

